X-ray Point Source Populations Constituting the Galactic Ridge X-ray Emission

Apparently diffuse X-ray emission has been known to exist along the central quarter of the Galactic Plane since the beginning of the X-ray astronomy, which is referred to as the Galactic Ridge X-ray emission (GRXE). Recent deep X-ray observations have shown that numerous X-ray point sources account for a large fraction of the GRXE in the hard band (2-8 keV). However, the nature of these sources is poorly understood. Using the deepest X-ray observations made in the Chandra Bulge Field (Revnivtsev et al., 2009,2011), we present the result of a coherent photometric and spectroscopic analysis of individual X-ray point sources for the purpose of constraining their nature and deriving their fractional contributions to the hard band continuum and Fe K\alpha line emission of the GRXE. Based on the X-ray color-color diagram, we divided the point sources into three groups: A (hard), B (soft and broad spectrum), and C (soft and peaked spectrum). The group A sources are further decomposed spectrally into thermal and non-thermal sources with different fractions in different flux ranges. From their X-ray properties, we speculate that the group A non-thermal sources are mostly AGNs and the thermal sources are mostly white dwarf (WD) binaries such as magnetic and non-magnetic cataclysmic variables (CVs), pre-CVs, and symbiotic stars, whereas the group B and C sources are X-ray active stars in flares and quiescence, respectively. In the log N-log S curve of the 2-8 keV band, the group A non-thermal sources is dominant above about 10^{-14} erg cm^{-2} s^{-1}, which is gradually taken over by Galactic sources in the fainter flux ranges. The Fe K\alpha emission is mostly from the group A thermal (WD binaries) and the group B (X-ray active stars) sources.

==> t04.tex <==
%\setlength{\tabcolsep}{0.01in}
\begin{deluxetable*}{ccccc}
\tabletypesize{\scriptsize}
\tablewidth{0pc}
\tablecolumns{5}
\tablecaption{Statistics of total, \textit{bright}, and variable sources\label{t04}}
\tablehead{
 \colhead{Group} &
 \colhead{$N$\tablenotemark{a}} &     
 \colhead{$N_{\textit{bright}}$\tablenotemark{b}} & 
 \colhead{$N_{\textrm{var}}$\tablenotemark{c}} &
 \colhead{$f_{\textrm{var}}$\tablenotemark{d}}
%
}
\startdata
Aa & 160 & 153 & 8 & 0.03\,$\pm$\,0.03\\
Ab & 448 & 32  & 3 & 0.18\,$\pm$\,0.10\\
B1 & 562 & 62 & 6 & 0.16\,$\pm$\,0.09\\
B2 & 804 & 108 & 17 & 0.26\,$\pm$\,0.06\\
\hline
Total & 1974 & 355 & 34 & --
\enddata
\tablenotetext{a}{Total number of sources.}
\tablenotetext{b}{Number of sources with more than 100 counts in each group.}
\tablenotetext{c}{Number of variable sources in each group.}
\tablenotetext{d}{Fraction of variable sources among those with KS test result.A 1$\sigma$ statistical uncertainty is given.}
\end{deluxetable*}

